Learning to Split for Automatic Bias Detection

Classifiers are biased when trained on biased datasets. As a remedy, we propose Learning to Split (ls), an algorithm for automatic bias detection. Given a dataset with input-label pairs, ls learns to split this dataset so that predictors trained on the training split cannot generalize to the testing split. This performance gap suggests that the testing split is under-represented in the dataset, which is a signal of potential bias. Identifying non-generalizable splits is challenging since we have no annotations about the bias. In this work, we show that the prediction correctness of each example in the testing split can be used as a source of weak supervision: generalization performance will drop if we move examples that are predicted correctly away from the testing split, leaving only those that are mis-predicted. ls is task-agnostic and can be applied to any supervised learning problem, ranging from natural language understanding and image classification to molecular property prediction. Empirical results show that ls is able to generate astonishingly challenging splits that correlate with human-identified biases. Moreover, we demonstrate that combining robust learning algorithms (such as group DRO) with splits identified by ls enables automatic de-biasing. Compared to previous state-of-the-art, we substantially improve the worst-group performance (23.4% on average) when the source of biases is unknown during training and validation.

==> sections/ack.tex <==
\section*{Acknowledgement}
Research was sponsored by the United States Air Force Research Laboratory and the United States Air Force Artificial Intelligence Accelerator and was accomplished under Cooperative Agreement Number FA8750-19-2-1000. The views and conclusions contained in this document are those of the authors and should not be interpreted as representing the official policies, either expressed or implied, of the United States Air Force or the U.S. Government. The U.S. Government is authorized to reproduce and distribute reprints for Government purposes notwithstanding any copyright notation herein.

==> tables/tox21.tex <==
\begin{table}[t]
\centering
\footnotesize
\caption{The splits learned by \texttt{ls} on property \texttt{NR.AR} correlates with other properties that are not given to the algorithm.
Specifically, \texttt{ls} allocates 58.3\% of the actives into the training split and 41.2\% of the actives into the testing split (top row). However, if we focus on the subset with \texttt{SR.ATAD5} active, this distribution shifts drastically to 17.1\% vs. 82.9\%.
}
\label{tab:ch4_tox21}
\begin{tabular}{lcc}
\toprule
                             & $\frac{ \text{\#\texttt{NR.AR} active in } \mathcal{D}^{\text{train}}}{\text{\#\texttt{NR.AR} active}}$
                             & $\frac{ \text{\#\texttt{NR.AR} active in } \mathcal{D}^{\text{test}}}{\text{\#\texttt{NR.AR} active}}$\\\midrule
All examples                 & 58.3\% &  41.6\% \\\midrule\midrule
Subset with \texttt{NR.AhR}       active & 13.0\% &  87.0\%	\\\midrule
Subset with \texttt{NR.AR.LBD}    active & 82.3\% &  17.7\%	\\\midrule
Subset with \texttt{NR.Aromatas}  active & 62.5\% &  37.5\%	\\\midrule
Subset with \texttt{NR.ER}        active & 64.0\% &  36.0\%	\\\midrule
Subset with \texttt{NR.ER.LBD}    active & 75.3\% &  24.7\%	\\\midrule
Subset with \texttt{NR.PPAR.gam}  active & 40.0\% &  60.0\%	\\\midrule
Subset with \texttt{SR.ARE}       active & 45.5\% &  54.6\%	\\\midrule
Subset with \texttt{SR.ATAD5}     active & 17.1\% &  82.9\%	\\\midrule
Subset with \texttt{SR.HSE}       active & 66.7\% &  33.3\%	\\\midrule
Subset with \texttt{SR.MMP}       active & 53.6\% &  46.4\%	\\\midrule
Subset with \texttt{SR.p53}       active & 45.2\% &  54.8\%	\\\bottomrule
\end{tabular}
\end{table}


